Spectral Rank Certification for Foundation Model Adapters

Nominal LoRA rank is a design parameter; calibrated spectral evidence is a separate inferential quantity. This article develops a finite-sample framework for inferring effective rank structure in public foundation-model adapters. The theoretical core is an exact chi-square divergence for the fixed-dimensional Gaussian rank-one reference experiment, with an unknown signal direction integrated under a rotation-invariant reference prior. The resulting series yields a computable finite-sample Le Cam bound at concrete layer sizes, an explicit remainder bound for numerical truncation, and the rectangular Baik-Ben Arous-Peche (BBP) limit. A compact-manifold Laplace expansion shows that finite-sample likelihood evidence also depends on leading spectral gaps through the factor $s_1^{|m-n|}\prod_{i\ge2}(s_1^2-s_i^2)$, motivating joint calibration of clustered singular values. Building on these results, we introduce an empirical-null workflow for PEFT LoRA adapters: factor reconstruction, Monte Carlo $p$-values, stagewise and block testing, and module-wise and corpus-level BH reporting. In an audit of 26 public adapters, 684 modules, six architecture families, and 31,770 public-checkpoint spectra rows, calibrated effective rank is typically much smaller than nominal rank and differs systematically from 95\% energy retention. A measured RoBERTa-RTE slice on $n=24$ examples illustrates the measurement path from calibrated ranks to task evaluation, without treating the slice as a utility study. The main empirical finding is that calibrated effective rank is usually far below nominal rank, and that energy retention and statistical surprise answer different questions.

==> data/evidence_provenance_summary.tex <==
\begin{tabular}{@{}P{.19\linewidth}P{.23\linewidth}P{.27\linewidth}P{.23\linewidth}@{}}
\toprule
Source & Paper artifact & Origin & Supported interpretation \\
\midrule
Reference calibration & Figures 1--4 and 6; synthetic calibration tables & Seeded Gaussian/spiked-matrix simulation and exact series & Theorem and calibration checks for the reference experiment \\
Null-pipeline stress tests & Pipeline calibration table & Seeded null-only and misspecified synthetic matrices & False-positive and misspecification diagnostics \\
Public adapter spectra & Figure 7; adapter manifest and spectral evidence tables & 26 pinned public repositories; 684 modules; 31770 spectra rows & Real weights-only LoRA factor spectra \\
Measured downstream evaluation & Table \ref{tab:downstream}; evaluation records & 4 CPU inference rows on a 24-example GLUE-RTE validation slice & Controlled task measurement for the rank-truncation path \\
Quoted model-card context & Observational metadata records & 3 model-card values copied as metadata & External context with explicit source labeling \\
Verification controls & Parser and calibration control rows & 12 generated code-path rows & Code-path verification separated from evidence summaries \\
\bottomrule
\end{tabular}


==> data/journal_gate_summary.tex <==
\begin{tabular}{@{}lr@{}}
\toprule
Gate item & Count/status \\
\midrule
Public-checkpoint repositories & 26 \\
Public-checkpoint module rows & 684 \\
Public architecture families & 6 \\
Measured downstream evaluations & 4 \\
Verification controls & 12 \\
Submission status & \texttt{submission\_ready\_empirical\_gate\_passed} \\
\bottomrule
\end{tabular}

